Investigating the Bulk Properties of Charged Particles in Different $\eta$ Bins Using a Modified Tsallis Model

This paper presents a comprehensive analysis of the double-differential $p_T$ distributions of charged particles in twelve distinct pseudorapidity regions of equal width in $pp$ collisions at center-of-mass energies of 0.9, 2.36, and 7 TeV. Utilizing the modified Tsallis function with mean transverse flow velocity, our study demonstrates a very good agreement between experimental data and the model employed. The fit quality is consistently high across all $p_T$ ranges, as assessed by Data/Fit panels accompanying each plot. Extracted parameters, including kinetic freeze-out temperature ($T_0$), transverse flow velocity ($\beta_T$), non-extensivity parameter ($q$) and mean transverse momentum $\langle p_T \rangle$ dependencies are shown on pseudorapidity ($\eta$) and collision energy ($\sqrt{s}$). $T_0$, $\beta_T$ and $\langle p_T \rangle$ exhibit a decreasing trend with increasing $\eta$ due to lower in energy transfer along high $\eta$ regions, while they show a heightened sensitivity to $\sqrt{s}$. $q$ increases with $\eta$, indicating a closer thermal equilibrium in mid-$\eta$ particles. The paper also explores correlations among these parameters, emphasizing relationships between $T_0$, $\beta_T$, $q$ and $\langle p_T \rangle$. Our study provides valuable insights into the thermal and dynamic characteristics of high-energy proton-proton collisions, contributing to the broader understanding of the bulk properties of nuclear matter produced in these interactions.

==> Tables.tex <==
%\begin{document}
\begin{table*}[t!]
\begin{center}
\caption{The values of free parameters, the normalization constant, $\chi^2$ and $ndof$ obtained through the fitting procedure of the experimental data with modified thermodynamically consistent Tsallis distribution function given in Eq. (\ref{Eq. 3}).}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{ccccccccc}
\hline
\hline
Energy & $\eta$ & $T_{0}$ (GeV/$c$) & $q$ & $\beta_T$ &$\langle p_T \rangle$ & $N_0$ & $\chi^2$ & $ndof$   \\
\hline
    & 0.1 & 0.06341$\pm$0.01786  & 1.14110$\pm$0.00150 & 0.32320$\pm$0.02616 & 0.4696$\pm$0.0102 & 2641.75508$\pm$115.8066  & 3.03651  &  11  \\
    & 0.3  & 0.06297$\pm$0.01522  & 1.14380$\pm$0.00170 & 0.31320$\pm$0.09503 & 0.4676$\pm$0.0101 & 2781.18218$\pm$112.1516  & 2.25321  &  11  \\
    & 0.5 & 0.06086$\pm$0.01348  & 1.15180$\pm$0.00160 & 0.30230$\pm$0.07868 & 0.4657$\pm$0.0104 & 3102.71456$\pm$147.7188  & 2.02530  &  11  \\
    & 0.7 & 0.05841$\pm$0.00800  & 1.15780$\pm$0.00210 & 0.29330$\pm$0.01027& 0.4594$\pm$0.0102 & 3505.54287$\pm$743.5215  & 0.79604  &  11  \\
    & 0.9 & 0.05607$\pm$0.01276  & 1.16250$\pm$0.00210 & 0.28230$\pm$0.08254 & 0.4505$\pm$0.0098 & 4164.10151$\pm$498.1546  & 2.33216  &  11  \\
900 GeV    & 1.1 & 0.05413$\pm$0.01093  & 1.16750$\pm$0.00170 & 0.27330$\pm$0.06171 & 0.4452$\pm$0.0096 & 4582.32914$\pm$483.4055  & 1.86525  &  11  \\
    & 1.3 & 0.05291$\pm$0.01811  & 1.16820$\pm$0.00160 & 0.26430$\pm$0.07412 & 0.4363$\pm$0.0097 & 5265.66198$\pm$926.7622  & 5.55728  &  11  \\
    & 1.5 & 0.05099$\pm$0.01561  & 1.17397$\pm$0.00190 & 0.25540$\pm$0.04437 & 0.4326$\pm$0.0098 & 5929.58665$\pm$986.7167  & 4.46334  &  11  \\
    & 1.7  & 0.04787$\pm$0.02216  & 1.18117$\pm$0.00170 & 0.24440$\pm$0.06597 & 0.4241$\pm$0.0095 & 7377.07226$\pm$774.4555  & 10.74392  &  11  \\
    & 1.9 & 0.04630$\pm$0.01999  & 1.18512$\pm$0.00220 & 0.23140$\pm$0.04048 & 0.4178$\pm$0.0097 & 8426.60004$\pm$647.9168  & 9.20621  &  11  \\
    & 2.1 & 0.04593$\pm$0.02960  & 1.18614$\pm$0.00210 & 0.22680$\pm$0.02826 & 0.4159$\pm$0.0098 & 8631.31528$\pm$988.5175  & 20.35876  &  11  \\
    & 2.3  & 0.04462$\pm$0.02712  & 1.18842$\pm$0.00180 & 0.21980$\pm$0.07804 & 0.4103$\pm$0.0096 & 9324.19040$\pm$959.5391  & 17.08767  &  11  \\
\hline
\hline
    & 0.1  & 0.06808$\pm$0.01862  & 1.13570$\pm$0.00120 & 0.35320$\pm$0.06337 & 0.4988$\pm$0.0132 & 2521.38642$\pm$632.14545  & 11.70458  &  11  \\
    & 0.3  & 0.06666$\pm$0.01492  & 1.14120$\pm$0.00110 & 0.34320$\pm$0.03279 & 0.4962$\pm$0.0131 & 2737.22202$\pm$721.88793  & 11.15294  &  11  \\
    & 0.5 & 0.06376$\pm$0.01681  & 1.14920$\pm$0.00140 & 0.33143$\pm$0.05559 & 0.4894$\pm$0.0130 & 3153.96261$\pm$744.76038  & 9.25049  &  11  \\
    & 0.7    & 0.06191$\pm$0.01356  & 1.15390$\pm$0.00150 & 0.32320$\pm$0.05177 & 0.4841$\pm$0.0130 & 3573.01903$\pm$419.57793  & 5.62341  &  11  \\
    & 0.9 & 0.06064$\pm$0.01133  & 1.16190$\pm$0.00140 & 0.31520$\pm$0.04847 & 0.4880$\pm$0.0129 & 3823.19530$\pm$3021.7187  & 7.87698  &  11  \\  
    & 1.1  & 0.05850$\pm$0.01103  & 1.16690$\pm$0.00130 & 0.30420$\pm$0.03436 & 0.4806$\pm$0.0128 & 4205.86453$\pm$2683.5818  & 5.04605  &  11  \\   
 2.36 TeV   & 1.3  & 0.05579$\pm$0.02381  & 1.17230$\pm$0.00140 & 0.29280$\pm$0.03592 & 0.4707$\pm$0.0127 & 5075.72273$\pm$440.52248  & 5.98253  &  11  \\
    & 1.5& 0.05365$\pm$0.01198  & 1.17960$\pm$0.00130 & 0.28350$\pm$0.03698 & 0.4683$\pm$0.0126 & 5756.07442$\pm$505.87002  & 10.42228  &  11  \\
    & 1.7 & 0.05025$\pm$0.00855  & 1.18650$\pm$0.00120 & 0.27510$\pm$0.02376 & 0.4585$\pm$0.0125 & 7189.78232$\pm$466.20394  & 2.77283  &  11  \\
    & 1.9 & 0.04862$\pm$0.007163  & 1.19260$\pm$0.00120 & 0.26805$\pm$0.04759 & 0.4577$\pm$0.0123 & 7994.20741$\pm$426.04139  & 3.75365  &  11  \\
    & 2.1  & 0.04630$\pm$0.007202  & 1.19160$\pm$0.00130 & 0.25152$\pm$0.06712 & 0.4367$\pm$0.0122 & 9987.74237$\pm$881.8848  & 8.32422  &  11  \\
    & 2.3 & 0.04509$\pm$0.0052719  & 1.20030$\pm$0.00130 & 0.23545$\pm$0.06614 & 0.4399$\pm$0.0121 & 10601.8529$\pm$1992.9341  & 10.56820  &  11  \\
\hline
\hline
    & 0.1   & 0.06832$\pm$0.01981  & 1.14680$\pm$0.00160 & 0.35330$\pm$0.15715 & 0.5197$\pm$0.0141 & 3032.5352$\pm$1322.6312  & 35.64743  &  11  \\
    & 0.3  & 0.06677$\pm$0.01563  & 1.15380$\pm$0.00150 & 0.34330$\pm$0.15345 & 0.5192$\pm$0.0140 & 3309.0728$\pm$1337.3670  & 31.29893  &  11  \\
    & 0.5  & 0.06402$\pm$0.01590  & 1.16380$\pm$0.00170 & 0.33232$\pm$0.14413 & 0.5172$\pm$0.0139 & 3791.2659$\pm$1332.9927  & 25.72337  &  11  \\
    & 0.7    & 0.06217$\pm$0.01108  & 1.16680$\pm$0.00180 & 0.32430$\pm$0.13194 & 0.5091$\pm$0.0140 & 4232.3776$\pm$1321.5200  & 18.98844  &  11  \\
    & 0.9  & 0.06081$\pm$0.01061  & 1.17180$\pm$0.00160 & 0.31552$\pm$0.13338 & 0.5068$\pm$0.0138 & 4620.0929$\pm$1306.8054  & 14.87211  &  11  \\
    & 1.1  & 0.05867$\pm$0.010235  & 1.17780$\pm$0.00190 & 0.30456$\pm$0.13057 & 0.5013$\pm$0.0138 & 5143.6981$\pm$1318.5732  & 13.59588  &  11  \\   
 7 TeV   & 1.3  & 0.05662$\pm$0.01019  & 1.18120$\pm$0.00180 & 0.29345$\pm$0.12279 & 0.4916$\pm$0.0137 & 5963.8385$\pm$119.83735  & 10.29492  &  11  \\
    & 1.5 & 0.05441$\pm$0.01071  & 1.18720$\pm$0.00200 & 0.28435$\pm$0.12457 & 0.4866$\pm$0.0139 & 6822.2853$\pm$1415.1623  & 8.82797 & 11 \\
    & 1.7 & 0.05060$\pm$0.01011  & 1.19840$\pm$0.00220 & 0.27576$\pm$0.12001 & 0.4824$\pm$0.0138 & 8452.8398$\pm$1587.1667  & 7.00883  &  11  \\
    & 1.9 & 0.04948$\pm$0.01015  & 1.20140$\pm$0.00210 & 0.27016$\pm$0.11475 & 0.4795$\pm$0.0135 & 9092.0292$\pm$1398.6969  & 5.97471  &  11  \\
    & 2.1   & 0.04853$\pm$0.01062  & 1.20410$\pm$0.00210 & 0.25262$\pm$0.12012 & 0.4725$\pm$0.0134 & 9961.0765$\pm$1431.1808  & 6.80707  &  11  \\
    & 2.3 & 0.04584$\pm$0.01077  & 1.20860$\pm$0.00230 & 0.24830$\pm$0.12475 & 0.4640$\pm$0.0134 & 11652.4080$\pm$1642.1596  & 10.65240  &  11  \\    
\hline
\end{tabular}
\end{adjustbox}
\end{center}
\end{table*}
%\end{document}

